Quantifying Memory Utilization with Effective State-Size

The need to develop a general framework for architecture analysis is becoming increasingly important, given the expanding design space of sequence models. To this end, we draw insights from classical signal processing and control theory, to develop a quantitative measure of \textit{memory utilization}: the internal mechanisms through which a model stores past information to produce future outputs. This metric, which we call \textbf{\textit{effective state-size}} (ESS), is tailored to the fundamental class of systems with \textit{input-invariant} and \textit{input-varying linear operators}, encompassing a variety of computational units such as variants of attention, convolutions, and recurrences. Unlike prior work on memory utilization, which either relies on raw operator visualizations (e.g. attention maps), or simply the total \textit{memory capacity} (i.e. cache size) of a model, our metrics provide highly interpretable and actionable measurements. In particular, we show how ESS can be leveraged to improve initialization strategies, inform novel regularizers and advance the performance-efficiency frontier through model distillation. Furthermore, we demonstrate that the effect of context delimiters (such as end-of-speech tokens) on ESS highlights cross-architectural differences in how large language models utilize their available memory to recall information. Overall, we find that ESS provides valuable insights into the dynamics that dictate memory utilization, enabling the design of more efficient and effective sequence models.

==> main_material/1_intro_old.tex <==
\RP{need help with intro + abstract sections + making punchlines + cutting things down heavily (and moving them to appdx.)}
\RP{Please flag things that could go to the appendix.}

\NT{How valuable are the boxes with high-level findings in the sections that are already quite concise, like the featurizer and initialization section. Seems like we're just wasting space there}

\RP{we could potentially remove them if we're really out of space, but i think it makes it easier to understand what's going on, since most things discussed in this paper are new for this field.}

% \RP{lets get a full draft done by Wed. @Neehal.} \NT{Sounds good}


\section{Introduction}
\label{sec:intro}

In recent years, the success of sequence models \citep{attention, s5, mamba} in the context of deep learning has largely been driven by advancements in architectures that are highly parallelizable, enabling efficient utilization of modern hardware accelerators like GPUs. Model parallelizability is a key characteristic that distinguishes these frameworks from other sequence models like RNNs and LSTMs \citep{rnn, lstm}.

\NT{Why are we talking about model parallelism? It is not relevant for us}

\RP{we have to somehow explain and motivate our scope of analysis, which are LIVs. The main difference between LIVs and other models is the fact that LIVs can be parallelized across sequence. RNNs can also be written as $y = Tu$ under some circumstances, so really the differentiating factor is this parallelizability.}

\MP{I think what we want to say here is that a successful architecture is built with computational units that are (a) high \textit{quality} -- in terms of performance -- and (b) run efficiently on hardware accelerators. For these reasons, we as a field have converged to particular computational units of a few different classes: convolutions, linear recurrences, and generalized structured operators.}

\MP{I think here, before we jump into our framework and why that enables the development of our own analysis tools, we should state what the problem we are trying to solve is (broadly). Here's a draft attempting to do it. [WHAT IS THE PROBLEM, WHY IS IT RELEVANT, WHY HASN'T IT BEEN SOLVED YET (brief summary of where previous methods fail)]

Due to the nonlinearity and diversity of operators used deep learning, extracting insights related their inner workings is challenging...
}

\MP{@Rom - we will reintroduce the necessary LIV ideas in this paper. Even though the other paper will be out by the time the review starts, we decided it would be safer for this to be self-contained (the arxiv release will rely more on the other paper, however)

With the aim to make progress on the development of generally applicable analysis tools for computational units, we ground our method in new abstractions. It turns out that a class of computational units of interest can all be formalized as \textit{linear input-varying systems} (LIVs)
\begin{equation*}
    y_i = \sum_{j\in[\ell]} T_{ij}(u)u_j,
\end{equation*}
generalizing the notion of adaptive, or \textit{data-controlled} operators to a broader class than described in \cite{hyena_hierarchy}. The framework of LIVs decouples the (potentially) nonlinear i.e., $T(u)$ and linear i.e., $Tu$  computation required to materialize and apply the operator. For these reasons, this formulation enables the applications of a wide array of analysis methods based on the theory of linear systems and linear operators

LIV systems include and generalize a diverse array of computational units commonly used in model architectures, whose class is defined by the structure of the operator $T$: convolutions [let's start citing properly from the 90s], linear recurrences [CIT], and various forms of other structured operators [CIT]
}
%

% recent work \citep{liv} has revealed that they can all be expressed by a common linear-like structure: $y = Tu$.

% In this formulation, \( u \) and \( y \) denote the input and output sequences, respectively, while \( T \) represents a (potentially input-dependent) causal operator that maps input sequences to output sequences. 

% This linear-like structure encompasses a diverse array of model architectures, including convolutions, linear/non-linear dynamical systems, and various forms of attention \citep{chenlinearsystem, 1dconv, attention, linear_attention, s4, s5, liquids4, hyena_hierarchy, mamba, gla}. Moreover, it not only facilitate parallelization but also enables the recognition of various structures within $T$, such as low-rank, Toeplitz, or semi-separable forms, that could be exploited for further improvements in their memory footprint and/or computational efficiency.

Importantly, the linear structure enables uniform analysis of various models by visualizing $T$, a method employed in several prior works \citep{hiddenattentionofmamba,attentionsink,massiveactivationsllm}. However, a significant drawback of this approach is that simple visualizations of $T$ alone, often fail to capture important properties that differentiate various models. 
Other approaches include computing the rank of $T$ \citep{efficiencyoftransformers,lowrank-mha}, but are often limited to a single model class and/or overlook the operator's causal nature, which could significantly affect its rank \citep{attention_rank_layernorm}.
To address these limitations, we propose casting all models of interest into an inherently causal dual formulation: linear-like recurrences, which is made possible by the operator-recurrence duality (see Section \ref{sec:op_rec_duality}). By recasting these models into a uniform formulation, we can directly compare key properties such as their state-size, providing an additional basis for analysis and comparison across different model architectures.

\NT{We lost the flow here, this transition is now disjoint from the last paragraph. We need to mention memory utilization before this paragraph}

\MP{Top paragraph can be cleaned up a bit. From here, a top down approach could sound better:

In this work, we focus on developing analysis metrics to investigate the memory capacity of model architectures...

Memory capacity is a key property of sequence models, as it is related to their ability to implement basic circuits such as in-context recall. Memory capacity also affects the memory footprint of a model during autoregressive inference, as is the case for example in linear recurrences... 
} \RP{Yeah this top-down approach looks good.}

As the computational demands of large-scale generative models continue to grow, the need for architectures that optimize the performance-efficiency trade-off has become paramount. A key factor associated with this trade-off is memory capacity\footnote{Here, we refer to ``memory" in the sense commonly associated with the ``state" of dynamical systems, as described by \cite{Willems1989}, as opposed to the notion of language models memorizing some fact encountered during training \citep{physicsofllms}.} which impacts both training and inference costs. This is especially pertinent in the case of linear recurrences like state-space models (SSMs), where the state size, a determinant of memory capacity, directly influences computational requirements. However, memory capacity alone can be misleading, as models with similar capacities may learn to utilize their available memory to varying degrees. Memory utilization, in contrast, offers a distinct perspective from memory capacity, providing insight into the differences between architectures that have comparable computational efficiency. Drawing from classical signal processing and control theory, we propose a metric called \emph{\textbf{effective state-size}} which can be extracted using the rank of specific submatrices of $T$. Effective state-size serves as a proxy for the memory utilization of linear input-varying systems, encompassing the entire set of models of practical interest in generative sequence modeling. As such, we find that we can use it as an analysis tool for a variety of causal sequence models (Figure \ref{fig:ess-overview}). 

In this work, we explore the application of this metric as a tool for analyzing and improving various aspects of modern sequence models. Our technical contributions can be summarized as follows:

\begin{itemize}
    \item We provide a theoretical derivation of the effective state-size in the context of both input-invariant and input-varying systems (Section \ref{sec:theory})
    \item \textcolor{red}{Fill in the rest of these bullet points later}
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{assets/ess_overview.pdf}
    \caption{An overview of the effective state-size metric and its various downstream applications. }
    \label{fig:ess-overview}
\end{figure}

\MP{We are missing punchlines for contributions. We do all this and where does that get us? Why should a reader care to continue reading?}

==> main_material/2_theory_old.tex <==
\section{Theory}
\label{sec:theory}

% --------------------- NOTES
%- What are LIVs, featurizers, and operators.
%- Quick notation
%- Relation between state-size and operator rank
%	- SSM -> Operator rank: Show how the state-size of an SSM determines the rank of $H_i$ (state-projection inner product dimension is $n_i$)
%	- Arbitrary operator -> LTV SSM: Show that you can realize a minimal LTV given an arbitrary operator
%		- So we define ESS as the state-size of these minimal systems
%		- Causal ESS is minimal with respect to the input-state-projection
%		- Non-causal ESS is minimal with respect to both the input-state projection and the state-output projection
%	- TSS > Causal ESS > Non-causal ESS
%- Computing ESS
%	- Tolerance: Counting the number of singular values of $H_i$ above a set tolerance.
%	- Perplexity: Computing the "effective rank" of $H_i$, which involves normalizing the singular values into a probability distribution, computing its entropy, then exponentiating it. 
%  
% --------------------- END NOTES

\RP{Will have to better structure them into theorems and lemmas. Also definition of MCS, TCS, and others are still messy.}

In this section, we establish the relationship between the state-size of a state-space model and the submatrix rank of the operator $T$. We demonstrate that for any causal, input-invariant operator $T$, its submatrix rank determines the minimal state-size required for an input-invariant linear recurrence to realize the same operation. We refer to this metric as the ``effective state-size" (ESS) of the operator, and show that even in the more complex case of input-varying operators, where the minimal state-size may be difficult to determine, the ESS metric remains valuable as it provides a reliable lower bound for the minimally realizable state-size.

Consider a general linear recurrence with state $s$,
\begin{equation}\label{eq:ssm}
\begin{aligned}
    s_{k+1} &= A_{k}s_{k} + B_{k}u_k \\
    y_{k} &= C_k s_k + D_k u_k,
\end{aligned}
\end{equation} 
where $(A_k \in \RR^{n_{k+1} \times n_k}, B_k \in \RR^{n_{k+1} \times d}, C_k \in \RR^{n_k \times d}, D_k \in \RR^{d \times d})_{k \in [\ell]}$ and $n_k$ is the state-size at time-step $k$. Unrolling the recurrence unveils the dual causal operator $T$, in which\footnote{The notation used in this paper can be found in Section \ref{sec:notation}},
\begin{equation}\label{eq:ssm2operator}
    T_{ij} = 
    \begin{cases}
        0 & i<j\\
        D_{i} & i=j \\
        C_i A_{i-1 ; j+1}B_j & i>j 
    \end{cases};
\end{equation}

We can decompose the operator where $i>j$ into causal and anti-casual parts,
\begin{equation} \label{eq:op_decomp}
    T_{i:, :i-1} \equiv H_i = \underbrace{\begin{bmatrix}
    C_{i} \\
    C_{i+1}A_{i} \\
    C_{i+2}A_{i+1; i}\\
    \vdots \\
    C_{\ell}A_{\ell -1 ; i}
    \end{bmatrix}}_{{\scriptsize \begin{gathered}
    d(\ell-i+1) \times n_i\\\textit{anti-causal}\end{gathered}}}
    \underbrace{\begin{bmatrix}
    A_{i - 1 ; 2}B_1  &
    A_{i-1 ; 3}B_2 &
    \dots & 
    A_{i-1}B_{i-2} & B_{i-1} 
    \end{bmatrix}}_{\scriptsize \begin{gathered}n_i \times d (i-1)\\\textit{causal}\end{gathered}} \equiv \mathcal{O}_i\mathcal{C}_i
\end{equation} 
for which, the causal term $\mathcal{C}$ (also known as the \textit{controllability matrix}), is the input-state projection matrix, i.e., $s_i = \mathcal{C}_iu_{:i}$, and likewise, the anti-causal term $\mathcal{O}$ (also known as the \textit{observability matrix}), is the state-output projection matrix.

Based on Equation \eqref{eq:op_decomp}, we can show the following relation between state-size and operator rank.
\begin{note}
\begin{lemma}\label{lemma:state_size_upper_bounds_rank}
The state-size of any model formulated with Equation \eqref{eq:ssm}, upper bounds the rank of its dual operator submatrix $H_i$ for each time-step $i$. I.e., $n_i \geq \rank(H_i)$.
\end{lemma}
\end{note}
\begin{proof}
    Equation \eqref{eq:op_decomp} establishes the relation that the state-size $n_i$, determines the inner product dimension of $H_i$'s decomposition, and therefore it subsequently is an upper bounds to rank of $H_i$.
\end{proof}
Next, we aim to demonstrate that the rank of $H_i$ determines the smallest possible state-size by first showing that any operator can be realized as a linear recurrence using arbitrary decompositions of $H_i$, then showing that 

Next, we demonstrate that the submatrix rank in fact indicates the minimally realizable state-size for linear time-varying systems as follows:
\begin{note}
    \begin{theorem}
        $\rank(H_i)$ determines the minimal state-size that is required for a time-varying recurrence to realize an identical input to output mapping ($y = Tu$). 
    \end{theorem}
\end{note}
\begin{proof}
For input-invariant operators, one can reformulate the state-projection matrices with arbitrary decompositions of $H_i$ to realize new recurrences (with possibly different state-sizes) using the realization algorithm described in Section \ref{sec:realize_recurrence}. Since $\rank(H_i)$ determines the minimum possible inner product dimension of $H_i$'s decomposition (Equation \eqref{eq:op_decomp}), it consequentially determines the minimum state-size that would be necessary to realize the equivalent operation.
\end{proof}

For input-invariant systems, the system features $(A_i, B_i, C_i, D_i)_{i \in [\ell]}$ themselves are not autoregressively computed from the inputs, therefore, one can reformulate the state-projection matrices with arbitrary decompositions of $H_i$ to realize a new recurrence (with possibly different state-sizes) without violating the causality of the system, using a realization algorithm described in Section \ref{sec:realize_recurrence}. 

\begin{theorem}
test
\end{theorem}
\begin{proof}
    test
\end{proof}

Since $\rank(H_i)$ determines the minimum possible inner product dimension of $H_i$'s decomposition, it consequentially determines the smallest state-size that would be necessary to realize the equivalent operation ($y = Tu$). Therefore, methods like SVD that could produce minimal decompositions could be used to construct minimal state-projection matrices that subsequently realizes minimal system features $(A_i^*, B_i^*, C_i^*, D_i^*)_{i \in [\ell]}$.

\begin{definition}[Effective State Size]
Despite a model actually materializing a user-defined state-size ($\tilde{n}$) during inference, its operation is effectively equivalent to that of a recurrence with state-size $n_i = \rank(H_i) \equiv n_i^*$. We therefore, define the ``\textit{effective state-size}" (ESS) metric at any time-step $i$ as the rank of the submatrix $H_i$.
\end{definition}

Now consider a general input-varying linear recurrence, where causal functions maps the input sequence into the system features (e.g., $f_A(u_1, \dots, u_k) \mapsto A_k$). Due to its input-dependence, the same minimal realization algorithm is not guaranteed to obtain a recurrence in which the features do not violate causality (i.e., $A_k^*$ depends on future inputs) and therefore is not viable for model-order reduction.
Nonetheless, the effective state-size metric could still be used as an analysis tool as the materialized state-size (MCS) -- defined through the model hyperparameters -- upper bounds it. Therefore, given any operator, one may safely assume that any recurrence with the equivalent operation must at least materialize a state-size greater than that indicated by the operator's ESS. This concept can be applied to make ESS-informed distillation 

then be applied to gain insights when comparing different model architectures, as well as provide heuristics in tasks such as model-order-reduction of state-space models.

\RP{also talk about TCS, MCS, ESS how are they different? what do they mean? relate them to cache-grouping like GQA, etc.}


\subsection{Computing Effective State-Size}

In practice, computing the ESS numerically involves selecting a tolerance value and counting the numerically computed singular values of $H_i$ ($\mathbf{\Sigma}_i$) above the set tolerance:
\begin{equation}
    n^{\star}_i \coloneqq |\{\sigma_i^m : \sigma^m_i > \tau,\; \sigma^m_i \in \mathbf{\Sigma}_i\}|.
\end{equation}
With Eckart–Young–Mirsky's theorem, one may interpret the tolerance-based ESS as the minimum required state-size of an input-invariant approximate operator for its reduced-order approximation error to be less than the set tolerance value.
\RP{@Stefano, can you check if this makes sense?}

One drawback of computing the tolerance based ESS is that it requires the somewhat aribtrary selection of the tolerance value itself. Alternatively, the tolerance values can be marginalized by computing the effective rank \cite{effective_rank}, which involves computing the exponentiated entropy (perplexity) of the normalize the singular values:
\begin{equation}
    \begin{gathered}
        p_i^m = \frac{\sigma_i^m}{\lVert \sigma_i\rVert_1}, \\
        n^{\dagger}_i \coloneqq \text{exp}\Big(-\sum_m p_i^m \log(p_i^m)\Big).
    \end{gathered}
\end{equation}
Unlike the tolerance-based discrete state-size metric, $n^{\dagger}$ can take values continuously ranging from 1 to $|\mathbf{\Sigma}_i|$. However, due to the normalization of singular values, the absolute values are discarded which may be important for some analyses. Moreover, computing the effective rank could pose numerical issues when the $p_i^m$ is close to 0 due to the logarithmic term. Nevertheless, both $n^\star$ and $n^\dagger$ could be used for model analysis, offering slightly different perspectives.

==> main_material/3_empirical_validation_old.tex <==
\section{Empirical Validation of Effective State-Size}
\label{sec:validation}

% \RP{main things we want to convey with this section are: 1. how our exp setup is broad enough to capture a wide variety of task and model space. 2. how ESS (per unit of task memory) is correlated to memory utilization as measured by synthetic tasks, and how that is not merely due to the fact that TSS is correlated to memory capacity.

% \begin{itemize}
%     \item Figure 2 (b) clearly shows that memory utilization is a better measure than memory capacity. 
%     \item We can create something like Figure 2 (a) but for TSS/TM for people to compare the plots, and put both of those in the appendix. \NT{yup, have a ton of plots that I'm tossing in appendix, this is one of them}
%     \item ESS/TSS vs TSS plot (state-utilization plot) is not as important as state-utilization as it depends on the task, but in the plot it's marginalized so it can go to the appendix. Figure 3 (d) is more informative for state-utilization.\NT{This is to show that there is ground to be gained in improving models since ESS scales sublinearly in TSS, but sure we can bail on it} \RP{But this is post-training anyways right? I think that would make sense for pre-training imo.} \NT{There's ground to be gained as in we should be able to train models that converge to higher state utilizations} \RP{Yes but conditioned on the fact that the task needs higher state-utilizations. So there's some conflationary aspect here, is what i'm trying to say.}
%     \item Fig 3 (c) accuracy vs state-utilization plot: state-saturation can be explained with the fact that \#kv is too large for its TSS. I think it has less to do with ESS, so could go to the appendix too. \NT{Yeah can probably toss this in appendix}
%     \item Fig 3 (a)/(b) (state-remembering/forgetting plot) this is a byproduct of ESS (per unit of task memory) being correlated with accuracy + state-collapse. So I would use it to support the correlation claim, but it doesn't have to be the main thing imo. \NT{I disagree. This is as important the cross-model correlation because of what I slacked you.} \RP{Okay, i'll wait till you're done writing the section and we can discuss further.}
% \end{itemize}

% In summary, i would just focus on conveying the fact that ESS is correlated with memory utilization as measured by synthetic tasks, and use all these plots as support for why they would be useful for further pre/mid/post-training analysis/applications.
% }

To demonstrate the practical utility of ESS beyond its theoretical interpretation discussed in Section \ref{sec:theory}, we next turn to an empirical analysis. In this section, we examine ESS across a wide range of tasks and models to understand how it varies across different regimes, with particular focus placed on its relationship with model performance on memory intensive tasks.

\textbf{Task space.} In order to explore ESS in an extensive, yet controlled manner, we iterate on a set of synthetic tasks proposed by \citet{mad} which have been shown to effectively approximate model performance on large-scale language tasks. Specifically, we train models on the MQAR, selective copying and compression tasks, each of which probe model skills related to recall -- a property of sequence models that requires high memory utilization and, consequently, high ESS. We note that here, we restrict the presentation of our results to MQAR and refer the reader to \ref{sec:extended_empirical_validation} for the results on selective copying and compression which showcase analogous trends.

\textbf{Model space.} We explore four models as is pertains to the scope of this analysis: gated linear attention (GLA), weighted linear attention (WLA), linear attention (LA) and softmax attention (SA). We chose this set of frameworks since, together, they capture a large portion of the space of modern sequence models. The key distinctions between these frameworks are as follows (more details can be found in Section \ref{sec:methods_formulation_featurizers}): 

\begin{itemize}[topsep=0pt]
    \item GLA layer: This layer implements the gated linear attention formulation described in \cite{gla}, where the recurrent feature $A$ (gating term) is input-varying, placing it in the same class as models like Liquid-S4 \citep{liquids4} and Mamba \citep{mamba}.
    \item WLA layer: This layer is nearly identical to GLA, but with an input-invariant $A$ matrix. This lies in the same class as frameworks like Hyena-S4D \citep{hyena_hierarchy}, RetNets \citep{retnet}, and gated-convolutions in general.
    \item LA layer: This layer is based off \cite{linear_attention}; $A$ is not trainable and is instead fixed as the identity matrix.
    \item SA layer: This is the canonical attention layer which is similar to linear attention, but with the addition of a softmax non-linearity applied to the attention matrix \citep{attention}, enabling unbounded TSS.
\end{itemize}

\paragraph{Experimental setup.} In our analysis, we exhaustively sweep across the tasks and models (which are comprised of two sequence mixing and two channel mixing layers) detailed above. Within each task, we also sweep across varying task difficulties. In the case of MQAR we do so by modulating the number of key-value (kv) pairs in the dataset as well as the sequence length of the data. Within each model, we sweep across varying TSS. For each task-model configuration, we compute the ESS and accuracy on a validation set every 10 epochs. We will refer to the entire space of task and models across which we sweep as the task-model space.
Finally, we split our profiling of ESS into two sections: cross task-model analysis (Section \ref{sec:cross_model}) and within task-model analysis (Section \ref{sec:within_model}). 

\subsection{Cross Task-Model analysis}
\label{sec:cross_model}
% \begin{figure}[H]
%     \centering
%     % Top plot (longer, at 90% text width)
%     \begin{minipage}[b]{0.9\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{assets/bivariate_kv_normalized_average_ess_all_models.pdf}  % Top plot
%         \label{fig:cross_model_plot}
%     \end{minipage}
    
%     % Vertical space between the top and bottom plots
%     \vspace{-0.6cm}
    
%     % Bottom plots (two smaller, centered at 45% width each)
%     \begin{minipage}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{assets/corr.pdf}  % Bottom left plot
%         \label{fig:corr_plot}
%     \end{minipage}
%     \hspace{0.1cm}  % Horizontal space between the two bottom plots
%     \vspace{-0.8cm}
%     \raisebox{0.15cm}{\begin{minipage}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{assets/average_univariate_Others_TSS_normalized_average_ess.pdf}  % Bottom right plot
%         \label{fig:state_utilization}
%     \end{minipage}}
%     \vspace{0.2cm}
%     \caption{(a) (b) (c) \NT{Tossing into appendix, so don't refer to it when writing}}
%     \label{fig:cross_correlation}
% \end{figure}


\begin{figure}[h] % set to [h] because [H} was wasting some space
    \centering
    % Top plot (centered at 65% width)
    \begin{subfigure}[b]{0.75\textwidth}
        \centering
        \includegraphics[width=\textwidth]{assets/bivariate_kv_normalized_average_ess_all_models.pdf}  % Top plot
        \vspace{-30pt}
        \caption{}
        \label{fig:cross_model_plot}
    \end{subfigure}
    \hspace{0.05cm}  % Slight horizontal space between the two plots
    % Bottom left plot (centered at 30% width)
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{assets/corr.pdf}  % Bottom left plot
        \vspace{-30pt}
        \caption{}
        \label{fig:corr_plot}
    \end{subfigure}
    \vspace{-15pt}
    \caption{(a) Scatter plots of accuracy vs ESS/kv across featurizers. Within each featurizer plot, all task-model configurations from the sweep corresponding to each featurizer are shown. (b) ESS/kv vs TSS/kv as a proxy for model performance as measured by correlation.}
\end{figure}


Our first goal is to understand how ESS correlates with performance on MQAR across the entire task-model space post-training. To appropriately analyze ESS across tasks, we need to normalize the metric against the memory demands of MQAR (refer to Section \ref{sec:methods_empirical_validation} for elaboration). To this end, we construct an adjusted form of ESS given by ESS/kv and compute correlation in this normalized space. 

\begin{myfindingbox}
Across the task-model space, ESS/kv and accuracy are positively correlated (Figure \ref{fig:cross_model_plot}), demonstrating the importance of memory utilization in recall-heavy tasks.
\end{myfindingbox}

As an aside, since SA performs very well in most of the task-model space due to its unbounded TSS, we restrict the remainder of our analysis to the recurrent frameworks and refer the reader to \ref{sec:extended_empirical_validation} for analogous results on SA. Next, to ensure that this correlation is not captured by memory capacity, we also analyze the correlation between TSS/kv and performance across models. 
\begin{myfindingbox}
For GLA, LA and WLA, the correlation between accuracy and ESS/kv is higher, substantiating ESS as a metric that captures aspects of model memory that TSS cannot (Figure \ref{fig:corr_plot}). 
\end{myfindingbox} 

\RP{I think we should somehow support the above claim with the within task-model results which demonstrates that ESS captures correlation even when TSS is fixed. I think it's stronger than saying that correlation is higher with ESS. Could be sth like "This substantiates ESS as a metric that captures aspects of model memory that TSS cannot. In the next section, we go further, and demonstrate that even under the same architecture (where TSS cannot capture inter-model variations), insightful correlations can be drawn by analyzing its ESS.". I'd also remove the "substantiating ESS as a metric that captures ..." in the finding itself, because that's not really a finding, it's more like our opinion that we draw from the finding.} \NT{I'm down for this}

%\RP{
%an attempt to clear up some logic that's still appears fuzzy to me, these are my opinions, let me know if you think it's wrong or irrelevant:
%
%\textbf{plot showing ess-accuracy correlation within a training run (for each task-model bucket).}
%\begin{itemize}
%    \item \textbf{does this motivate pre-training analysis?} to motivate looking at ESS during init we need correlation between initial ESS vs final performance (or some other metric that is associated with good performance). So in a fuzzy sense yes? but would be better if we just directly correlated initial ess to final performance (and maybe we'll find regimes for which it makes sense to do pre-training analysis). 
%    \item \textbf{does this motivate mid-training analysis?} In some ways, yes because it literally is mid-training analysis, so if we get anything valuable from it, it does motivate to further pursue mid-training analysis. Also, if we see some weird anomalies due to state-collapse, that motivates looking at ess mid training (but i think we can show something like this with ESS vs epoch plots over models that had final performances of close to 0\%, because for plots that run into state-collapse, i believe there's not much of a signal that makes ESS-acc correlation relevant since acc is around 0\%) Also the state-utilization/accuracy vs TM plot already showss state-collapse pretty well.
%    \item \textbf{how is this correlation metric useful/valuable?} It supports the fact that task memory impacts the ESS trajectory. So it supports us using ESS/kv metric over raw ESS metric, which is very important. Also would like to point out that we dont need to coin new terms like state-remembering/forgetting. 1. remembering/forgetting sounds like Mamba/S6's selective state stuff (so it comes with an additional baggage to define it accurately) 2. different choices on tolerance gets us different state-remembering/forgetting metrics and so explaining anything using state remembering/forgetting of a single selected tolerance gives us a very narrow story. 
%    
%    What we want to show here is the pattern in which low kv + high TSS leads to the model utilizing less states across the course of training relative to the case in which the task has high kv + low TSS; that holds individually across a wide range of tolerance values for the tol-ESS metric as well as with the entropy ESS metric. This finding basically supports the choice of using ESS/kv over raw ESS as mentioned previously, and there's no need to actually coin new terms to explain this phenomenon.
%\end{itemize}
%
%\textbf{plots showing state-utilization vs tm and accuracy vs tm}
%\begin{itemize}[noitemsep]
%    \item \textbf{does this motivate mid-training analysis?} yes, it shows state-collapse pattern for larger kv on GLA and WLA, but not for LA, motivating us to look at ESS throughout the course of training. These plots are very informative (would like to also see std or min/max values though)
%\end{itemize}
%
%\textbf{plot showing accuracy vs state-utilization (across task buckets?)}
%\begin{itemize}[noitemsep]
%    \item \textbf{how is this metric useful/valuable?} According to neehal, it shows that there there are grounds for improving state-utilization. But this is only relevant if the task requires high state-utilization in the first place, so there's a conflationary aspect in showing acc vs state-utilization of all model-task buckets together in a single plot. 
%    
%    If we our goal is to explain how there's ground for improving state-utilization (such as when state-collapse happens), we have to instead highlight the fact that there are models with low performance which are not due to limited memory capacity, but due to limited state-utilization. We can use this limited state-utilization phenomenon to motivate further investigation of ESS during training, by saying that it's likely due to trainability issues, or some other factor during training.
%
%    On the other hand, if our goal is to show how you can detect state-saturation (when ESS $\approx$ TSS) to prompt an increase in TSS for improving performance on the task, then we need to show cases where state-utilization is maxed out but has low performance, then show that with a higher TSS, the state-utilization is lower but it performs better. 
%    
%    \textbf{But I think for both of these points, the previous plot is clearer.}
%\end{itemize}
%
%\textbf{what i think is missing}
%\begin{itemize}
%    \item Missing clear motivation for pursuing pre-training analysis. It's not absolutely necessary to motivate pre-training analysis because the results we already obtained in the pre-training section speaks for itself, but, if we can show correlations across a larger model/task range that motivates further investigation of ESS pre-training, the story would be more compelling)
%\end{itemize}
%
%I think that's it, the rest looks great!
%}
%
%\NT{I agree with everything you wrote above. Let's bail on state forgetting and remembering and just focus on state saturation and mostly state collapse. We can place the focus mostly on state-collapse since that occurs in high TSS high KV regime which is where all of our downstream analyses are in and unlike state saturation is a solvable problem with ESS. For motivating pre-training analysis, yeah if you could make the plot on post-training ESS that would be great. However, just with respect to the plots here, there are a couple ways to motivate it: one, by virtue of LA not have a decaying A, it has higher ESS at initialization. It also performs best in state-collapse regime so it's reasonable to believe that higher ESS initializers are better. Two, there is the general idea in ML that where you start ends up being close to where you end. We want to end at high ESS to solve tasks that tend to result in state collapse so we want to see what happens when we start higher}
%
%\RP{Okay, i like the idea you have for motivating pre-training.}

\subsection{Within Task-Model Analysis}
\label{sec:within_model}

\begin{figure}[H]
    \centering
    
    % First row of plots
    \begin{subfigure}[b]{0.62\textwidth}
        \centering
        % \begin{picture}(0,0)
        %     \put(-10, 130){\textbf{(a)}}  % Custom coordinates for the label
        % \end{picture}
        \includegraphics[width=\textwidth]{assets/average_univariate_TSS_kv_correlation_average_ess_epoch_10.pdf} 
        \vspace{-25pt}
        \caption{}
        \label{fig:ess_training_plot}
    \end{subfigure}
    \hspace{0.1cm} % Horizontal space between the two top plots
    \begin{subfigure}[b]{0.36\textwidth}
        \centering
        \includegraphics[width=\textwidth]{assets/accuracy_utilization_plot.pdf}  % Top right plot
        \vspace{-25pt}
        \caption{}
        \label{fig:state_collapse_plot}
    \end{subfigure}
    \vspace{-15pt}
    \caption{(a) Correlation between ESS and accuracy over course of model training bucketed by TSS and kv. (b) Accuracy and state utilization as a function of kv for low and high TSS models.}
    \label{fig:within_correlation}
\end{figure}

While the previous findings support the utility of the ESS metric, the scope of the claims is restricted to correlations across task-model space. Note that such relationships fail to capture the following, equally important aspect of the metric: for a fixed model and task, how does performance evolve with ESS over the course of training? To understand the  dynamics of ESS in this context, we compute correlations between ESS and accuracy on a per-model, per-task basis over the course of training. Interestingly, we find that trends emerge when bucketing the task-model space on TSS and kv. 
\RP{Also here, i think we can mention the fact that we wanna know if ESS is useful where TSS can't be useful (since this is an iso-architecture analysis).} \NT{Yeah valid}

\begin{myfindingbox}
For less memory-intensive tasks trained using a high TSS, we observe a lower correlation between ESS and performance as opposed to the more memory-intensive tasks trained using a lower TSS (Figure \ref{fig:ess_training_plot}).
\end{myfindingbox}

This is in line with the interpretation of ESS as a measure for memory utilization. For easier tasks that are learned by a model with high memory capacity, the model is not incentivized to increase its memory utilization beyond where it resides at initialization. In contrast, for difficult tasks that operate in a memory constrained regime, the model is forced to increase its memory utilization in order to learn, resulting in strong positive correlations between accuracy and ESS over training. 

Digging a bit deeper, we further find that this form of ESS analysis reveals two failure modes of model learning: state saturation and state collapse. State saturation refers to the scenario in which a model has insufficient TSS to learn a task, resulting in its ESS converging near its TSS. This is reflected in its ESS/TSS (which we refer to as state utilization) converging near 1. We observe this in Figure \ref{fig:state_collapse_plot} where we note that models with a TSS of $8$ perform worse on the task as its difficulty scales due to a saturated state. State collapse, on the other hand, refers to the scenario in which a model has sufficient TSS to learn a task but its ESS fails to increase during training, resulting in a heavily underutilized state. With respect to state collapse, we observe the following:

\begin{myfindingbox}
For GLA and WLA, state collapse occurs in the high KV, high TSS bucket of task-model space where as for LA it does not (Figure \ref{fig:state_collapse_plot}). 
\end{myfindingbox}

While state saturation can only be solved by increasing TSS, state collapse can in principle be solved by increasing ESS. Unlike TSS which is a fixed hyperparameter of the model, one can modulate ESS by changing various aspects of the model pipeline. Even beyond the state collapse regime, given the positive correlation between ESS and performance across a vast task-model space, increasing ESS is a generally viable approach to improving model performance without sacrificing efficiency. We explore this idea in the results to follow.

% \paragraph{ESS concepts.} Here, we outline various ESS concepts we use to qualify changes in ESS over the course of model training. First, we introduce the terms \emph{\textbf{state remembering}} and \emph{\textbf{state forgetting}}, where the former refers to learning driven by increases in ESS and the latter refers learning driven by decreases in ESS. We further these concepts by investigating two failure modes of learning in the state remembering paradigm. These failure modes are termed \emph{\textbf{state saturation}} and \emph{\textbf{state collapse}} respectively. State saturation refers to the scenario in which a model has insufficient TSS to learn a task, resulting in its ESS converging near its TSS (i.e. state utilization close to 1). State collapse, on the other hand, refers to the scenario in which a model has sufficient TSS to learn a task via state remembering, but instead its ESS decreases significantly during training resulting in a heavily underutilized state (i.e. state utilization close to 0). We will explore each of these concepts and the regimes in which they arise in Section \ref{sec:intra_model}.



==> main_material/4_1_pretraining_analysis.tex <==
\subsection{Initialization-Phase Analysis}
\label{sec:pre_training}

Initialization in weight space plays a crucial role in machine learning, significantly impacting model convergence and training stability \citep{weight_init}. We extend this concept to the initialization of recurrent models in state space, leaning on the intuition from Figure \ref{fig:cross_model_plot} that suggests higher ESS can enhance performance. Namely, we illustrate how ESS at initialization can be used to inform featurizer selection -- the selection of the function that maps the input to the operator $T=f(u)$ or equivalently the recurrent features $(A_i(u_{:i}), B_i(u_{:i}), C_i(u_{:i}), D_i(u_{:i}))_{i \in [\ell]}$ -- and initialization schemes. In doing so, we uncover design flaws of a prominent model, S6 (Mamba) \citep{mamba}.

\begin{figure}[t] % would rather put this on top because there are plots for other sections here; I moved distillation figure
     \centering
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=.78\textwidth]{assets/ess-tss_scaling_all.pdf}
         %\vspace{0.5mm}
         \vspace{-15pt}
         \caption{} \label{fig:ess_vs_tss_scaling}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{assets/tss_vs_ess_expand_k_sweep_mean.pdf}
         \vspace{-27pt}
         \caption{}
         \label{fig:gla_mqar_vs_tss}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{assets/tss_vs_ess_vs_acc_arange_norm_sweep_mean.pdf}
         \vspace{-27pt}
         \caption{}
         \label{fig:arange_sweep}
     \end{subfigure}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{assets/distillation_loss_corr_single.pdf}
         \vspace{-27pt}
         \caption{}
         \label{fig:ess_distillation_loss_correlation_single}
     \end{subfigure}
     \vspace{-10pt}
     \caption{(a) ESS-TSS scaling in the S6, GLA and GLA-S6 featurizers. (b) ESS and accuracy on MQAR as a function of TSS in GLA. (c) ESS and accuracy on MQAR as a function of normalization factor for initialization in GLA-S6. (d) Distillation loss vs ESS of the teacher model.}
\end{figure}
% Refer to Figure \ref{fig:ess_distillation_loss_correlation} for additional results.
\paragraph{ESS-informed featurizer selection.}

To study the relationship between memory capacity and memory utilization in S6, we remove the short convolutional layer in the Mamba block and stack two of these modified blocks between SwiGLUs \citep{gluvariants}. Under the default MQAR task settings outlined in \cite{mad} (see Tables \ref{tab:pretraining_gla_hparams}, \ref{tab:pretraining_s6_hparams}, and \ref{tab:featurizer_mqar_settings} for details), we observe that S6 is entirely unable to learn MQAR (accuracy $\approx$ 0) across multiple scales of TSS (16 - 256) as shown in Figure \ref{fig:s6_loss_curves}. This aligns with results from \cite{deltanet}, which independently demonstrate the poor performance of S6 without the additional short convolutional layer on a different in-context recall task. To investigate the cause, we look into how S6 is preconditioned to utilize its memory by computing its ESS when processing a Gaussian noise input, prior to training.

\begin{myfindingbox}
Figure \ref{fig:ess_vs_tss_scaling} demonstrates that the ESS of S6 layers at initialization scales poorly with respect to TSS, notably failing to increase monotonically. In contrast, GLA layers \citep{gla}, configured with hyperparameters to match the TSS, model width, number of layers, and hidden-state normalization of the S6 model (see Section \ref{sec:methods_formulation_featurizers} and Table \ref{tab:pretraining_gla_hparams}), exhibit greater and monotonically increasing ESS-TSS scaling at initialization (Figure \ref{fig:ess_vs_tss_scaling}). 
Despite the architectural similarities between the S6 and GLA layers, Figure \ref{fig:gla_mqar_vs_tss} demonstrates that, unlike S6, GLA achieves accuracy improvements that correlate with increases in both TSS and ESS.
\end{myfindingbox}
% We observe even higher degrees of correlation in an alternative MQAR setting, shown in Figure \ref{fig:gla_mqar_vs_tss_custom}.
Based on these findings, we conjecture that the poor ESS-TSS scaling of S6 prevents the model from effectively utilizing all of its states, irrespective of increases in memory capacity.

\paragraph{ESS-informed initialization scheme.}

To further investigate the differences between the aforementioned S6 model and GLA model, we construct a composite model termed GLA-S6. This model adopts the feature-sharing structure of GLA (dividing dimensions into heads and sharing computations within a head), but applies the S6 featurization to the $A$ matrix as follows:
\begin{align}
    &\text{GLA (original): } &&A = \text{diag}(\text{sigmoid}(Wu)^{1/\beta}) \\
    &\text{GLA-S6: } &&A = \text{diag}(\text{exp}(-([1/\alpha \quad 2/\alpha \quad \dots \quad n/\alpha]^T \odot \text{softplus}(Wu)))).
\end{align}
Like S6, GLA-S6 fails to learn MQAR across the same range of TSS (see Figure \ref{fig:s6_loss_curves}) and exhibits poor initialization-ESS scaling as shown in Figure \ref{fig:ess_vs_tss_scaling}. Upon further inspection, we identify the cause of poor ESS scaling: with each new state introduced, the \texttt{arange} term ($[1 \quad 2 \quad \dots \quad n]$) exponentially pushes new entries of $A$ towards zero, negating the effects of additional states despite the increase in TSS. Therefore, to ameliorate the poor ESS scaling, we propose a simple solution: increase the normalization factor.
\begin{myfindingbox}
By scaling the normalization factor ($\alpha$), Figure \ref{fig:arange_sweep} shows that GLA-S6 achieves improvements in MQAR accuracy post-training, reflecting the impact of increasing its initialization-ESS, despite the models having identical memory capacities.
\end{myfindingbox}

These experiments demonstrate the efficacy of analyzing ESS at initialization, as they reveal how different models are preconditioned to utilize their working memory. This analysis helps identify potentially weak featurization and initialization schemes, enabling us to pinpoint shortcomings in the S6 featurizer and implement a straightforward fix.
%Since a lot more can happen during training, next we turn to the analysis of memory utilization during training.

==> main_material/5_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\NT{Personally don't think we need a separate section dedicated to this. We can just note the limitations in related works or conclusion so we don't detract from our method too much}

==> supplementary_material/_reproducibility.tex <==
\section*{Impact Statement}
% this section doesn't count towards page limit

This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.


